Deep Extrinsic Manifold Representation for Vision Tasks

Non-Euclidean data is frequently encountered across different fields, yet there is limited literature that addresses the fundamental challenge of training neural networks with manifold representations as outputs. We introduce the trick named Deep Extrinsic Manifold Representation (DEMR) for visual tasks in this context. DEMR incorporates extrinsic manifold embedding into deep neural networks, which helps generate manifold representations. The DEMR approach does not directly optimize the complex geodesic loss. Instead, it focuses on optimizing the computation graph within the embedded Euclidean space, allowing for adaptability to various architectural requirements. We provide empirical evidence supporting the proposed concept on two types of manifolds, $SE(3)$ and its associated quotient manifolds. This evidence offers theoretical assurances regarding feasibility, asymptotic properties, and generalization capability. The experimental results show that DEMR effectively adapts to point cloud alignment, producing outputs in $ SE(3) $, as well as in illumination subspace learning with outputs on the Grassmann manifold.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );sub makeexternaldocument {if (!($root_filename eq $_[0])){system( "latexmk -cd -pdf \"$_[0]\"" );}
}

==> parts/exp.tex <==
\section{Experiments}
\label{sec:exp}




In this section, we demonstrate the effectiveness of applying extrinsic embedding to deep learning settings on two representative manifolds in computer vision.
%The first task is to estimate relative motion between two point clouds on affine transformation group $SE(3)$, and the second is to estimate illumination subspaces as Grassmann manifold $\mathcal{Gr}(m, \mathbb{R}^n)$. 
The experiments are conducted from several aspects below:
\begin{itemize}
    \item Whether DEMR takes effects in improving the performance of certain tasks?
    \item Whether the geometrical structure boosts model performance facing unseen cases, \eg, the ability to extrapolate training set.
\item Whether extrinsic embedding yields valid geometrical restrictions.
\end{itemize}
 The validations are conducted on two canonical manifold applications in computer vision
\subsection{Task I: affine motions on $SE(3)$}
\label{sec:exp1}
Estimating the relative position and rotation between two point clouds has a wide range of downstream applications. 
The reference and target point clouds 
 $P_R, P_t \in \mathbb{R}^{N\times3}$ are in the same size and shape, with no scale transformations.
The relative translation and rotation can be arranged separately in vectors 
or together in a matrix lying on $SE(3)$.
%and each relative spatial relationship lies on the manifold $SE(3)$. \vspace{-0.5cm}
\subsubsection{Experimental Setup}
\paragraph{Training Detail}
During training, at each iteration stage, a randomly chosen point cloud from $2,290$ airplanes is transformed by randomly sampling rotations and translations in batches. The rotations are sampled according to the models, \ie, the models producing axis angles are fed with rotations sampled from axis angles, and so on. 
%Then the pairs are fed into the models and output the transformations in corresponding representations. %All the models are compared after 650000 iterations of training. 
%

% Comparison metrics
\paragraph{Comparison metrics}
To validate the ability of the model to preserve geometrical structures, geodesic distance is the opted metric at the testing stage. 
\cite{zhou2019continuity,levinson2020analysis_svd} uses minimal angular difference to evaluate the differences between rotations, 
which is not entirely compatible with Euclidean groups, since it calculates the translation part and rotation part separately. 
For two rotations $R_1, R_2$ and $R' = R_1R_2^{-1}$ with its trace to be $tr(R')$, there is $L_{angle}=\cos^{-1}((tr(R')-1)/2)$.
For intrinsic metric, the geodesic distance between 
two group elements are defined with Frobenius norm for matrices
 $d_{int}(M_1, M_2)= \|\log(M_1^{-1}M_2)\|$, 
 where $\log(M_1^{-1}M_2)$ indicates the logarithm map on the Lie group.
 For extrinsic metric, we take Mean Squared Loss (MSE) between $J_{SE}(M_1)$ and $J_{SE}(M_2)$.
% \vspace{-0.4cm}
\begin{table}[H]
\centering
\caption{On the task of estimating relative affine transformations on $SE(3)$ for point clouds, the results are reported by the geodesic distance between the estimation and the ground truth. The best results across models are emphasized, where the smallest errors come from extrinsic embedding.}
\begin{tabular}{c|ccc}
    \toprule
    Mode&avg&median&std\\
    \midrule
         euler&26.83 & 15.54&32.23\\
         axis&31.96 & 10.66&27.75\\
         6D&10.28 &\textbf{5.36}&\textbf{21.54} \\
         9D&\textbf{10.23} &6.09&25.30\\
     \bottomrule  
    \end{tabular}
\label{tab:full_SE3}
% \vspace{-0.5cm}
\end{table}
% \end{wraptable} 
 For models with Euler angle and axis-angle output,  the predicted rotation and translation are organized in Euclidean form, and they are reorganized into Lie algebra $se(3)$. Finally, the distances are calculated in $SO(3)$ by exerting an exponential map on their $se(3)$ forms.
 %

 
\paragraph{Architecture detail}
%
Similar as \cite{zhou2019continuity,levinson2020analysis_svd}, 
the backbone for point cloud feature extraction is composed of 
a weight-sharing Siamese architecture containing two simplified PointNet Structures \cite{qi2017pointnet}
$\Phi_i:\mathbb{R}^{N\times3}\rightarrow \mathbb{R}^{1024}$
where $i=1,2$. 
After extracting the feature of each point with an MLP, 
both $\Phi_1$ and $\Phi_2$ utilize max pooling to produce a single vector $z_1, z_2$ respectively, 
as representations of features across all points in $P_r, P_t$. Concatenating $z_1, z_2$ to be $z$, 
another MLP is used for mapping the concatenated feature to the final higher-order Euclidean representation 
$Y_{\mathbb{E}}$. 
%
Finally, Euler angle quaternion coefficients and axis-angle representations will be directly obtained from the last linear layer of the backbone network of dimension, $3, 3, 4$ respectively.
For manifold output, the $SE(3)$ representation will be given by both cross-product and SVD, with details in Supplementary materials.
%
The translation part is produced by another line of $\mathtt{fc}$ layer of 3 dimensions.
 Because MSE computation between 
two isometric matrices are based on each entry,  total MSE loss is the sum of rotation loss
 and translation loss.
% Moreover, for the rotation matrix of dimension 3, 
% with the differentiable SVD operation in Pytorch,
%  the inverse of extrinsic embedding
%  computation takes negligible time compared to the whole pipeline.
%
\paragraph{Estimation accuracy and conformance}
To validate the necessity of structured output space, 
firstly we compare the affine transformation estimating network 
with different output formations. 
The translation part naturally takes the form of a vector 
and the rotation part can be in the form of Euclidean representations 
%like Euler-angle, Axis-Angle, 
and $SO(3)$ in matrix forms.
%such as 6D cross product representation and 9D SVD representation.
%
The dataset is composed of generated point cloud pairs with random transformations, where the rotations are uniformly sampled from various representations, namely, Euler angle, axis-angle in $3$-dimensional vector space, and $SO(3)$. The translation part is randomly sampled from a standard normal distribution. 

The advantage of manifold output produced by baseline DEMR is revealed in Table \ref{tab:full_SE3} and Figure \ref{fig:percentile}, output via extrinsic embedding takes the lead across three statistics.
\begin{figure}[H]
    \centering
\includegraphics[scale=1,bb=0 0 50 50]{pics/result_full.png} 	
    \caption{The cumulative distributions comparison of position errors for the pose regression task on $SE(3)$.}
	\label{fig:percentile}
\end{figure}

\begin{table*}
    \centering
    \small
    \caption{Comparison of different embeddings. DEMR takes the lead in predicting accuracy, with two types of embedding functions, namely, 6D and 9D.  Even when the ratio of unseen cases increases, DEMR has better performance all along.}
    \scalebox{0.85}{
    \begin{tabular}{c|ccccccccccccccc}
    \toprule
    &  
    \multicolumn{3}{c}{10\%}&\multicolumn{3}{c}{20\%}&\multicolumn{3}{c}{40\%}&\multicolumn{3}{c}{60\%}&\multicolumn{3}{c}{80\%}\cr
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
    &avg&med&std &avg&med&std &avg&med&std &avg&med&std &avg&med&std\cr
        euler & 77.81&54.42&77.52 &35.58&13.07&48.94 &28.82&17.02&30.89&27.22&16.27&35.52 &27.22&16.27&31.75 \\
        axis &75.57 &50.71 &78.60 &36.95 &12.38 &54.40&20.73&12.51&27.63&21.95&12.75&27.15&18.96&10.66&24.75\\
        6D&71.09&\textbf{29.39}&80.09&\textbf{17.12}&\textbf{5.25} &40.54&\textbf{10.85}&\textbf{5.07}&\textbf{19.60}&\textbf{9.76}&\textbf{4.93}&\textbf{19.60}&10.29&\textbf{5.01}&\textbf{21.08} \\
        9D&\textbf{70.72}&30.99 &\textbf{63.18}&19.83&5.62&\textbf{39.22}&12.91&6.28&22.66&12.24&6.40&24.18&\textbf{10.23}&5.31&22.60 \\
    \toprule
    \end{tabular}
    }    
    \label{tab:generalization}
\end{table*}
%%% Table for Grassmann
\begin{table*}
    \centering
        \small
        \caption{Test result reported in average $D_{\mathcal{G}}$ with an example result of a test sample, and the epoch at which the model converged.}
    % \scalebox{0.77}{
    \begin{tabular}{c|ccc}
    \toprule
        Input & GrassmannNet \cite{lohit2017dl_mani} & DIMR & DEMR\\
        \midrule

         \begin{minipage}
         [b]{0.3\columnwidth}
		\centering
		\raisebox{.2\height}{scale=1,bb=0 0 30 30]{pics/B13.jpeg}}
        \end{minipage}  
        &
         \begin{minipage}
         [b]{0.3\columnwidth}
		\centering
		\raisebox{.2\height}{scale=1,bb=0 0 30 30]{pics/GrassmannNet.jpeg}}
        \end{minipage}
        &
        \begin{minipage}
         [b]{0.3\columnwidth}
		\centering
		\raisebox{.2\height}{\includegraphics[scale=1,bb=0 0 30 30]{pics/DIL_B13.jpeg}}
        \end{minipage}  
        &
        \begin{minipage}
         [b]{0.3\columnwidth}
		\centering
		\raisebox{.2\height}{\includegraphics[scale=1,bb=0 0 30 30]{pics/DEL_B13.jpeg}}
        \end{minipage}  
\\
        avg $D_{\mathcal{G}}(U_{gt}, U_{out})$& 9.6826& 3.4551&3.4721 \\
     epoch & 320 & 680&140\\
     
    \bottomrule   
    \end{tabular}
    %}
    \label{tab:grassresult}
    %\vspace{-0.5cm}
\end{table*}
% %


\paragraph{Generalization ability}
To evaluate DEMR over its improvement in generalization ability in comparison with unstructured output space, the training set 
only contains a small portion of the whole affine transformation space while the test set encompasses affine transformations 
sampled from the whole rotation space.
To be fair in the sampling step across the compared representations, the sampling process is conducted uniformly in 
the representations spaces respectively.  
 %
 For models with axis-angle and Euler angle output, the input point cloud pair is constructed with rotation representation whose entries
  sampled $\mathrm{iid}$ from Euclidean ranges.
 For Euler representations, the lower bounds of the ranges are  $\pi$, 
 and the upper bounds are $\pi$ multiplied by $90\%, 80\%, 60\%, 40\%,20\%$, 
 while the test set is sampled from $[-\pi, \pi]$. 
 %
 The training set with axis-angle representations is also obtained by sampling Euclidean ranges. 
 %
 When constructing a training set on $SO(3)$, the uniform sampling process is conducted in the same way with axis-angle sampling, the segments are taken in ratios in the same way with the two aforementioned settings,  and then exponential mapping is used to yield random samples on $SO(3)$.
%
Facing unseen cases, DEMR has better extrapolation capability compared to plain deep learning settings with unstructured output space.  
As shown in Table \ref{tab: generalization}, results from deep extrinsic learning show great competence despite the portion size of the training set. 
% From Figure \ref{fig:avg} to Figure \ref{fig: std}, the gap of generalization ability magnifies when the training set becomes more limited, while DEMR has better performance.

\subsection{Task II: illumination subspace, the Grassmann manifold}
Changes in poses, expressions, and illumination conditions are inevitable in real-world applications,
but seriously impair the performance of face recognition models.
%
It is universally acknowledged that an image set of a human face under different conditions
 lies close to a low-dimensional Euclidean subspace. 
%specially for different illuminations the ill-posed inverse problem is to compute illumination subspace.
%As analyzed in \cite{lohit2017dl_mani}, 
After vectorizing images of each person into one matrix in dataset Yale-B \cite{YaleB}, 
experiments reveal that the top $d=5$ principal components (PC) generally capture more than $90\%$ of the singular values.
%as shown in Figure \ref{}.%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%bububu%%%%%%%%%%%%%%%%%%% 
%Therefore the eigenvectors of top PCs can be a concise summarization of representational illumination patterns across different individuals. 
%Apparently for a resized image of size $s\times s$, the linear space spanned by these top eigenvectors forms an illumination subspace on $\mathcal{G}(d, \mathbb{R}^{s^2})$.
% Therefore the illumination subspace refers to the linear span of these eigenvectors.
%\subsubsection{Problem Formulation}
As an essential application of DEMR, we take the feature extraction CNN as $T(\cdot)$ in Equation \ref{eq: combination}.
in high-dimensional Euclidean space, and obtain the final result by
inversely mapping the estimation to the Grassmann manifold.

\subsubsection{Experimental Setup}
\paragraph{Architectural detail}
A similar work sharing the same background comes from \cite{lohit2017dl_mani}, which assumes the output of the last layer in the neural network to lie on the matrix manifolds or its tangent space. We take GrassmannNet in the former assumption in \cite{lohit2017dl_mani} as the baseline, where the training loss function is set to be Mean Squared Loss. For all the models to be compared, the ratio of the training set is $0.8$, and all of the illumination angles are adopted.
In addition, the data preparation step also follows \cite{lohit2017dl_mani},  and other training details are recorded in supplementary materials.  
% 这里补充
On extended Yale Face Database B, each grayscale image of $168\times192$ is firstly resized to $256\times256$ as the input of CNN, while for subspace ground truth, they are resized to $28\times28=784$ for convenience of computation.  
 %Based on Lambertian model \cite{belhumeur1998illumin_cone}, Images of a convex object with Lambertian reflectance is a convex polyhedral cone in $\mathbb{R}^n$, and a query image in the illumination cone can be reconstructed via $\mathcal{I} = \max(Bs,0)$ to filter out the negative values,  with $\mathcal{I}$ being the reconstructed image, $B$ being an illumination basis and $s$ the lighting coefficients. Our task is to 
 \paragraph{Dataset processing}
The input face image $I_i^j$ indicates the $i_{th}$ face under the $j_{th}$ illumination condition, where $j=1,\ldots, 64$ for Yale B dataset.  If we adopt the top $d$ PCs, the output is assumed to be in the form of $\{E_i^1, E_i^2,\ldots, E_I^d\}$, $k=1\ldots, d$ and $<E_i^k, E_i^l>=\delta_{kl}$ where $\delta_{kl}$ is a Kronecker delta function. Each PC is rearranged as a vector, thus $vec(E_i^k)$ is of size $784\times1$ and we define $U_i = [vec(E_i^1), vec(E_i^2) \ldots vec(E_i^d)]$, and the output of the network is $U_iU_i^T$.
%Then the desired estimator  $F:\mathbb{R}\rightarrow \mathcal{G}(d, \mathbb{R}^{784})$ yields the equivalent class $[U_i]$ under the equvalance relation $U_i\sim U_iQ$, for any unit orthogonal transformation $Q$. Given image $I_i^j$, our task is to predict the illumination subspace $U_i$.
Most of the intrinsic distances defined on the Grassmannian manifold are based on principal angles (PA), for $P_1, P_2\in \mathcal{G}(m, \mathbb{R}^n)$,
with SVD $P_1^{T}P_2=USV^{T}$ where $S=diag\{cos(\theta_1),cos(\theta_2),\ldots,cos(\theta_m)\}$, PAs of Binet-Cauchy (BC) distance is $1-\Pi_{k=1}^K\cos^2\theta_k$ 
%on basis $1-(det(P_1^TP_2))$ 
and PAs of Martin (MA) distance is $\log\Pi_{k=1}^K(\cos^2\theta_k)^{-1}$.
For comparison of effectiveness and training advantage,  the deep intrinsic learning takes $D_{\mathcal{G}}(U_{gt}, U_{out}) = $ as both the training loss and testing metric, where $U_{gt}$ and $U_{out}$ indicate the ground truth and the network output respectively.



\paragraph{Estimation accuracy and conformance}
The results of illumination subspace estimation are given in Table \ref{tab:grassresult}. Measured by the average of geodesic losses, DEMR architecture achieves nearly the same performance as DIMR while drastically reducing training time till convergence. 
With batch size set to be 10, we record training loss after every 10 epochs and report approximately the epoch at which the training loss converged in the third row in Table \ref{tab:grassresult}.
Besides, both DIMR and DEMR surpass GrassmannNet in the task of illumination subspace estimation, and DEMR still takes fewer epochs for training than GrassmannNet.
In the first row of Table \ref{tab:grassresult}, on one of the test samples, the results from GrassmannNet, DIMR, and DEMR are displayed. In addition, the conformance of extrinsic and intrinsic metrics can be referred to as supplementary materials.
% \vspace{-0.3cm}

